Inductive Attention for Video Action Anticipation

Anticipating future actions based on spatiotemporal observations is essential in video understanding and predictive computer vision. Moreover, a model capable of anticipating the future has important applications, it can benefit precautionary systems to react before an event occurs. However, unlike in the action recognition task, future information is inaccessible at observation time -- a model cannot directly map the video frames to the target action to solve the anticipation task. Instead, the temporal inference is required to associate the relevant evidence with possible future actions. Consequently, existing solutions based on the action recognition models are only suboptimal. Recently, researchers proposed extending the observation window to capture longer pre-action profiles from past moments and leveraging attention to retrieve the subtle evidence to improve the anticipation predictions. However, existing attention designs typically use frame inputs as the query which is suboptimal, as a video frame only weakly connects to the future action. To this end, we propose an inductive attention model, dubbed IAM, which leverages the current prediction priors as the query to infer future action and can efficiently process the long video content. Furthermore, our method considers the uncertainty of the future via the many-to-many association in the attention design. As a result, IAM consistently outperforms the state-of-the-art anticipation models on multiple large-scale egocentric video datasets while using significantly fewer model parameters.

==> exclude.tex <==
\begin{algorithm}[t]
\caption{Refresh Algorithm for Indexed Memory}\label{alg:memory}
\begin{algorithmic}
\State Given an indexed memory $M_t \in \{M^K_t, M^V_t\}$ in key-value pair, and a predefined maximal memory capacity $C$.
\If{length of $M_t > C$ }
    \If{refresh}
        \State $(p^K, p^V) \gets \texttt{pop}(M_t)$ {\color{gray}\scriptsize \Comment{key-value of pop element.}}
        \State $corr \gets softmax(\frac{(p^K)^T (M^K_t)}{\sqrt{d}})$
        \State $M^V_t \gets \frac{M_t^V + corr \cdot p^V}{1+corr}$ {\color{gray}\scriptsize \Comment{update memory values.}}
    \Else
        \State $\texttt{pop}(M_t)$
    \EndIf
\EndIf
\State \textbf{return} $M_t$
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{img/memory_fresh_new.png}
    \caption{Memory refresh. The popped element distributes its content $p^V$ to the activated memory slots by comparing its key $p^K$ and the memory key $M^K_t$. The refresh function is deterministic and parameter-free.}
    \label{fig:refresh_mem}
\end{figure}


To alleviate the information loss due to limited memory length, we propose a refresh algorithm to distribute the content of the popped element to activated memory. For example, assume $p^K,p^V$ are the key and value of the popped element, and $M^K_t, M^V_t$ are the keys and values of the still active memory. The refresh algorithm performs the following update for each timestep $t$ when all memory slots are filled:
\begin{align}
score = softmax(\frac{(p^K)^T (M^K_t)}{\sqrt{d}}) \label{eq:refresh_1} \\
Refresh(p^K, p^V, M^K_t, M^V_t) = \frac{score \cdot p^V + M_t^V}{1+score} \label{eq:refresh_2}.
\end{align}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{img/supervision_scheme.png}
    \caption{Different supervision scheme demonstration with example activity. \textbf{The left scheme} takes the target action at the fixed time point as the learning target consistently. \textbf{The right scheme} anticipates the next action $\tau_a$ steps ahead for every step. Such a difference makes the anticipation model trained in the right scheme capable of performing in the continuous inference scenario.}
    \label{fig:supervision_scheme}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{img/augmentation.png}
    \caption{Jitter sampling augmentation replaces each video frame $x_t$ in the train sequence by randomly drawing a source frame from the video segment enclosed by $x_{t-1}$ and $x_t$. The first frame (i.e., $x_{t-8}$ in the figure) keeps intact to prevent crossing the video boundary.}
    \label{fig:augmentation}
\end{figure}

The ablation study shows that incorporating memory refresh can mitigate the negative impact on model performance when memory capacity is limited. It may benefit cases when the computing resource is constrained, e.g., when used for online inference. Memory update policy and refresh algorithm are shown in Figure~\ref{fig:refresh_mem} and Algorithm~\ref{alg:memory}.

Comparing the numbers under the same input length but different in memory capacities, it can be seen that memory capacity is roughly the bottleneck of model performance. For example, about 17.0 MT5R is obtained with the memory capacity set to 10 seconds, regardless of the length of inputs. Also, with sufficient memory capacity, the model can achieve about 17.3-17.5 MT5R.


Memory refresh can mitigate performance gaps arising from insufficient memory capacity. However, an exception occurs when using 60-second inputs together with 30-second memory, which could be related to the unbalanced composition of actions in the input activity and further mislead the model due to the older context. Memory refresh even makes the specific case worse since eq~(\ref{eq:refresh_1}) always injects the completely discarded element (i.e., summed to 1 in $score$) to the activated memory cells. Indeed, a potential improvement in memory design is possible by introducing an advanced topology, such as a graph or hierarchy structure, embedded with sophisticated memory management. We leave this aspect for future work.
